Tilted discs in six poorly studied cataclysmic variables

In this work, we search for negative superhumps (nSHs) in poorly studied cataclysmic variables using TESS data. We find three eclipsing binaries with nSH signatures: HBHA 4204-09, Gaia DR3 5931071148325476992, and SDSS J090113.51+144704.6. The last one exhibits IW And-like behaviour in archival ZTF data, and appears to have shallow, grazing eclipses. In addition, we detect nSH signatures in two non-eclipsing systems: KQ Mon and Gaia DR3 4684361817175293440, by identifying the orbital period from the superorbital-dependent irradiation of the secondary. We discover nSH signatures in one more system, [PK2008] HalphaJ103959, by using an orbital period from another work. An improved mass ratio - nSH deficit relation $q(\varepsilon_-)$ is suggested by us, which agrees with independent measurements on nova-like variables. With this relation, we estimate the mass ratios of all systems in our sample, and determine the orbital inclinations for the three that are eclipsing. All systems with discovered nSHs in this work are excellent targets for follow-up spectroscopic studies.

==> Tilted discs in six poorly studied CVs/figures/ebsummary.tex <==
\begin{figure}
    \centering
    \includegraphics{images/ebsummary.pdf}
    \caption{Orbital phase curves of Table~\ref{tab:ebList} systems.
    Light curves were smoothed by a fourth-order Savitzky-Golay filter
    of window size 10~d before folding. Orbital phases are offset with
    +0.50 for the sake of clarity.}
    \label{fig:ebsummary}
\end{figure}

==> Tilted discs in six poorly studied CVs/figures/irradiation.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/irradiation.png}
    \caption{A model CV system at an orbital phase
    $\varphi_\text{orb}=0.5$, as it would be seen by an observer. Four
    precession phases $\varphi_\text{prec}$ of a disc with tilt
    $\theta=6\degr$ are illustrated. The orbital plane of the system is
    defined by dotted lines. It divides space into two half-spaces: the
    near (above the plane) and the far one (below the plane), with
    respect to the observer. The precession phase is defined such that
    the system is the brightest at \mbox{$\varphi_\text{prec} = 0$}. In
    this orientation, the disc has the largest projected area at
    \mbox{$\varphi_\text{prec}=0$}. Conversely, at
    \mbox{$\varphi_\text{prec} = 0.5$}, it has the smallest projection,
    but faces towards the secondary and irradiates it the most.
    \citet{Kimura2021}, Figure 9 gives a full description of CV
    configurations in titled-disc regimes.} 
 \label{fig:irradiation}
\end{figure}

==> Tilted discs in six poorly studied CVs/figures/qeps.tex <==
\begin{figure*}
\centering
\includegraphics{images/qeps.pdf}
\caption{Different $q(\varepsilon_-)$ relations against NL variables
with $\varepsilon_-,q$ measurements from Table \ref{tab:stars_q_e}. (a)
Solid line: \citet{Montgomery2009}, Dashed line: \citet{Wood2009}. Both
relations underestimate $q(\varepsilon_-)$ for given measurements. (b)
Dotted line: Equation \eqref{eq:Warner1995final}, derived from the
approximation by \citet{Warner1995} used in Equation
\eqref{eq:epsilon-q_relation}. This fails to accurately describe
\citet{Paczynski1977} in $q$ regimes near 0.7. Blue curve: a computed
$q(\varepsilon_-)$ relation from our treatment in Section
\ref{sec:Discussion_massratio} that makes use of \citet{Paczynski1977}.
Shaded region: solutions between $R_d=$0.9--1.1$r_\text{tidal}$. All
measurements belong to this region within uncertainty.}
\label{fig:qeps}
\end{figure*}

==> Tilted discs in six poorly studied CVs/figures/star03summary.tex <==
\begin{figure*}
    \centering
    \includegraphics{images/star03summary.pdf}
    \caption{Photometry and analysis of \mbox{HBHA 4204-09}. (a)
    Long-term photometry from: \mbox{ASAS-SN $g$} (purple downward
    triangles), \mbox{ASAS-SN $V$} (green upward triangles). Temporal
    coverage of TESS: Sector 15 (light blue), Sector 16 (yellow). (b)
    Residual (mean-subtracted) SAP flux from TESS data. (c) Associated
    LS periodogram of (b), with indications of
    $P_\text{prec},P_\text{orb},P_\text{nSH}$ signals from Table
    \ref{tab:shList} (blue dashes). (d)--(g) Binned orbital profiles
    around disc precession phases \mbox{$\varphi_\text{prec}= 0.00,
    0.25, 0.50, 0.75$} with nSH subtraction (blue squares) and without
    one (black circles). The typical standard deviation of data in bins
    is 25 \electronpersecond. This system has a high inclination, and
    the parts of the secondary in both half-spaces are accessible to the
    observer. The secondary is expected to be the most irradiated in
    panels (d) and (f), where the observed out-of-eclipse profile is
    non-flat. In panels (e) and (g), where no irradiation of the
    secondary is expected, the out-of-eclipse profile is mostly flat.}
    \label{fig:star03summary}
\end{figure*}


==> Tilted discs in six poorly studied CVs/figures/star04special.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{images/star04special.pdf}
    \caption{
    Z Cam-like episodes of Gaia-468436 in
    \mbox{ASAS-SN $g$} (blue downward triangles) and 
    \mbox{ASAS-SN $V$} (green upward triangles). 
    The Z Cam behaviour begins after a $\sim0.5$~mag fall in brightness. Emerging oscillations have a variable amplitude of $\sim 0.8$~mag and are quasi-periodic with $P \sim 20$~days. At about BTJD 1500, a brightening takes place, which is followed by a standstill at a level of 15.0~mag. At about BTJD 1760, the standstill is replaced with another oscillatory episode that has outbursts of similar period and amplitude as the former ones. No more Z~Cam episodes were observed in Gaia-468436 in this data.} 
 \label{fig:star04special}
\end{figure*}

==> Tilted discs in six poorly studied CVs/figures/star04summary.tex <==
\begin{figure*}
    \centering
    \includegraphics{images/star04summary.pdf}
    \caption{Photometry and analysis of \mbox{Gaia-468436}. (a)
    Long-term photometry from: \mbox{ASAS-SN $g$} (purple downward
    triangles), \mbox{ASAS-SN $V$} (green upward triangles). Temporal
    coverage of TESS: Sector 28 (light blue). (b) Residual
    (mean-subtracted) SAP flux from TESS data. (c) Associated LS
    periodogram of (b), with indications of
    $P_\text{prec},P_\text{orb},P_\text{nSH}$ signals from Table
    \ref{tab:shList} (blue dashes). (d)--(g) Binned orbital profiles
    around disc precession phases \mbox{$\varphi_\text{prec}= 0.00,
    0.25, 0.50, 0.75$} with nSH subtraction (blue squares) and without
    one (black circles). The typical standard deviation of data in bins
    is 4 \electronpersecond. The effect of variable irradiation in
    panels (d)--(g) is similar to the one observed in KIC~9406652
    \citep{Kimura2021}.}
    \label{fig:star04summary}
\end{figure*}


==> Tilted discs in six poorly studied CVs/figures/star08summary.tex <==
\begin{figure*}
    \centering
    \includegraphics{images/star08summary.pdf}
    \caption{Photometry and analysis of \mbox{KQ Mon}. (a) Long-term
    photometry from: \mbox{ASAS-SN $g$} (purple downward triangles),
    \mbox{ASAS-SN $V$} (green upward triangles). Temporal coverage of
    TESS: Sector 34 (light blue). (b) Residual (mean-subtracted) SAP
    flux from TESS data. (c) Associated LS periodogram of (b), with
    indications of $P_\text{prec},P_\text{orb},P_\text{nSH}$ signals
    from Table \ref{tab:shList} (blue dashes). (d)--(g) Binned orbital
    profiles around disc precession phases \mbox{$\varphi_\text{prec}=
    0.00, 0.25, 0.50, 0.75$} with nSH subtraction (blue squares) and
    without one (black circles). The typical standard deviation of data
    in bins is 16 \electronpersecond. The blue and the black curves
    differ due to the significant nSH contribution to the observed
    system flux. In blue curves of different $\varphi_\text{prec}$,
    there seems to be a change of shape and amplitude near
    $\varphi_\text{orb} = 0.5$, which is expected, but could be also due
    to noise. \citet{Kimura2021} provide models for such orbital curves
    that could explain these observations.}
    \label{fig:star08summary}
\end{figure*}

==> Tilted discs in six poorly studied CVs/figures/star13special.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{images/star13special.pdf}
    \caption{IW~And episodes of SDSS-090113 in \mbox{ZTF $g$} (teal
    circles) and \mbox{ZTF $r$} (magenta diamonds). Three seasons of
    photometry are shown. The first season starts with oscillations that
    are terminated by brightening. This is one of the defining features
    of the IW~And phenomenon \citep{Kato2019,KatoASAShrana2022}. The
    second season shows the beginning of a new oscillatory episode that
    is variable in amplitude. The episode continues in the third season
    and abruptly ends at BTJD 2315.}
 \label{fig:star13special}
\end{figure*}

==> Tilted discs in six poorly studied CVs/figures/star13summary.tex <==
\begin{figure*}
    \centering
    \includegraphics{images/star13summary.pdf}
    \caption{Photometry and analysis of \mbox{SDSS-090113}. (a)
    Long-term photometry from: ASAS-SN $g$ (purple downward triangles),
    ASAS-SN $V$ (green upward triangles), Catalina  $V$ (pink squares).
    Temporal coverage of TESS: Sector 44 (light blue), Sector 45
    (yellow), Sector 46 (light blue). (b) Residual (mean-subtracted) SAP
    flux from TESS data. (c) Associated LS periodogram of (b), with
    indications of $P_\text{prec},P_\text{orb},P_\text{nSH}$ signals
    from Table \ref{tab:shList} (blue dashes). Data from (b) was
    smoothed by a fourth-order Savitzky-Golay filter of window size 10 d
    before constructing the periodogram. This was done solely for the
    sake of clear identification of $P_\text{prec}$ by the reader, and
    not for periodicity measurements. (d)--(g) Binned orbital profiles
    around disc precession phases \mbox{$\varphi_\text{prec}= 0.00,
    0.25, 0.50, 0.75$} with nSH subtraction (blue squares) and without
    one (black circles). The typical standard deviation of data in bins
    is 4 \electronpersecond. SDSS-090113 appears to have shallow grazing
    eclipses that are barely detectable for some $\varphi_\text{prec}$.
    Observed eclipses vary in depth and width for different
    $\varphi_\text{prec}$. This could be explained by a secondary that
    partially covers the tilted disc only when the projected area of the
    disc is large.}
    \label{fig:star13summary}
\end{figure*}

==> Tilted discs in six poorly studied CVs/figures/star14summary.tex <==
\begin{figure*}
    \centering
    \includegraphics{images/star14summary.pdf}
    \caption{Photometry and analysis of \mbox{Gaia-593107}. (a) Residual
    (mean-subtracted) SAP flux from TESS data. (b) Associated LS
    periodogram of (a), with indications of
    $P_\text{prec},P_\text{orb},P_\text{nSH}$ signals from Table
    \ref{tab:shList} (blue dashes). (c)--(f) Binned orbital profiles
    around disc precession phases \mbox{$\varphi_\text{prec}= 0.00,
    0.25, 0.50, 0.75$} with nSH subtraction (blue squares) and without
    one (black circles). The typical standard deviation of data in bins
    is 8 \electronpersecond. Similar to the other eclipsing binaries in
    our sample, the secondary is expected to be the most irradiated in
    panels (c) and (e), where the observed out-of-eclipse profile is
    non-flat. In panels (d) and (f), these profiles are mostly flat, and
    the system brightness does not seem to increase near
    $\varphi_\text{orb} = 0.5$.}
    \label{fig:star14summary}
\end{figure*}

==> Tilted discs in six poorly studied CVs/figures/star15summary.tex <==
\begin{figure}
    \centering
    \includegraphics{images/star15summary.pdf}
    \caption{Photometry and analysis of \mbox{PK-103959}. (a) Long-term
    photometry from: ASAS-SN $g$ (purple downward triangles), ASAS-SN $V$
    (green upward triangles), Catalina  $V$ (pink squares). Temporal
    coverage of TESS: Sector 36 (light blue), Sector 37 (yellow). (b)
    Residual (mean-subtracted) SAP flux from TESS data. (c) Associated
    LS periodogram of (b), with indications of
    $P_\text{prec},P_\text{orb},P_\text{nSH}$ signals from Table
    \ref{tab:shList} (blue dashes).}
    \label{fig:star15summary}
\end{figure}

==> Tilted discs in six poorly studied CVs/tables/Stars_q_eps.tex <==
\begin{table*}
\caption{
A list of NLs with independently measured superhump deficit
$\varepsilon_{-}$ and mass ratio $q$. Equatorial coordinates come from
Gaia DR3 and are in the J2000 epoch. Other references:
($a$) \citet{Gies2013};
($b$) \citet{Africano1978};
($c$) \citet{Smak2019};
($d$) \citet{Subebekova2020};
($e$) \citet{Skillman1995};
($f$) \citet{Bruch2022};
($g$) \citet{Rodriguez-Gil2020};
($h$) \citet{Kozhevnikov2007};
($i$) \citet{Araujo-Betancor2003};
($j$) \citet{Boyd2017};
($k$) \citet{XiaoanWu2002};
($l$) \citet{Huber1998};
($m$) \citet{Taylor1998};
($n$) \citet{HoardSzkody1997};
($o$) \citet{Patterson1999};
($p$) \citet{Arenas2000};
($q$) \citet{PetersThorstensen2006};
($r$) \citet{Patterson1997};
($s$) \citet{Neustroev2011};
($t$) \citet{deMiguel2016};
($u$) \citet{Szkody1993};
($v$) \citet{Bruch2023};
($w$) \citet{Gulsecen2009};
($x$) \citet{Hellier1993};
($y$) \citet{Bruch2022}.
}

\label{tab:stars_q_e}
\begin{tabular}{lrrllll}
\multicolumn{1}{c}{Name} &
\multicolumn{1}{c}{RA} &
\multicolumn{1}{c}{Dec} &
\multicolumn{1}{c}{$q$} &
\multicolumn{1}{c}{$P_\text{orb}$} &
\multicolumn{1}{c}{$P_\text{nSH}$} &
\multicolumn{1}{c}{$|\varepsilon_{-}|$}

\\\hline

KIC 9406652 &
$ 19\h 31\m    29\fs    15$ &
$+45\degr 59' 06\farcs 1$ &
$^a0.83\pm0.07$ &
$^a0.25450(2)$ &
$^a0.23971(2)$ &
$0.0581(1)$ \\[0.5ex]

RW Tri &
$ 02\h 25\m    36\fs    16$ &
$+28\degr 05' 50\farcs 9$ &
$^d0.60\pm0.03$ &
$^b0.23188324(4)$ &
$^c0.2203(14)$ &
$0.050(6)$ \\[0.5ex]

MV Lyr &
$ 19\h 07\m    16\fs    29$ &
$+44\degr 01' 07\farcs 9$ &
$^e0.43^{+0.19}_{-0.13}$ &
$^e0.1329(4)$ &
$^f0.12816(1)$ &
$0.036(3)$ \\[0.5ex]

KR Aur &
$ 06\h 15\m    43\fs    92$ &
$+28\degr 35' 08\farcs 6$ &
$^g0.39^{+0.03}_{-0.04}$ &
$^g0.16277164(5)$ &
$^h0.1571(2)$ &
$0.035(1)$ \\[0.5ex]

DW UMa &
$ 10\h 33\m    52\fs    88$ &
$+58\degr 46' 54\farcs 7$ &
$^i0.39\pm 0.12$ &
$^i0.136606499(3)$ &
$^j0.132626(9)$ &
$0.02914(7)$ \\[0.5ex]

TT Ari &
$ 02\h 06\m    53\fs    08$ &
$+15\degr 17' 41\farcs 9$ &
$^k0.19\pm0.04$ &
$^k0.1375504(17)$ &
$^f0.132921(2)$ &
$0.03366(2)$ \\[0.5ex]

V592 Cas &
$ 00\h 20\m    52\fs    22$ &
$+55\degr 42' 16\farcs 2$ &
$^l0.19^{+0.10}_{-0.09}$ &
$^m0.115063(1)$ &
$^m0.11193(5)$ &
$0.0272(4)$ \\[0.5ex]

BH Lyn &
$ 08\h 22\m    36\fs    05$ &
$+51\degr 05' 24\farcs 6$ &
$^n0.45^{+0.15}_{-0.10}$ &
$^n0.15587520(5)$ &
$^o0.1490(11)$ &
$0.044(7)$ \\[0.5ex]

V603 Aql &
$ 18\h 48\m    54\fs    64$ &
$+00\degr 35' 02\farcs 9$ &
$^p0.24\pm0.05$ &
$^q0.13820103(8)$ &
$^r0.1341(3)$ &
$0.030(2)$ \\[0.5ex]

UX UMa &
$ 13\h 36\m   40\fs   95$ &
$+51\degr 54' 49\farcs 4$ &
$^s0.43\pm0.07$ &
$^t0.19667118(19)$ &
$^t0.186700(11)$ &
$0.05070(6)$ \\[0.5ex]

AY Psc &
$ 01\h 36\m   55\fs   46$ &
$+07\degr 16' 29\farcs 3$ &
$^u0.45\pm0.2$ &
$^v0.217320654(4)$ &
$^w0.20645(75)$ &
$0.050(3)$ \\[0.5ex]

TV Col &
$ 05\h 29\m   25\fs   53$ &
$-32\degr 49' 03\farcs 9$ &
$^x0.75\pm0.15$ &
$^y0.22860010(2)$ &
$^y0.215995(1)$ &
$0.055140(4)$ 


\end{tabular}
\end{table*}

==> Tilted discs in six poorly studied CVs/tables/ebList.tex <==
\begin{table*}
\caption{List of discovered eclipsing variables with no superhump
signatures. Equatorial coordinates come from Gaia DR3 and are in the
J2000 epoch.}
\label{tab:ebList}
\begin{tabular}{lrrcl}
\multicolumn{1}{c}{Name} &
\multicolumn{1}{c}{RA} &
\multicolumn{1}{c}{Dec} &
\multicolumn{1}{c}{TESS Sector} &
\multicolumn{1}{c}{P$_{\text{orb}}$}\\ \hline
TYC 8920-22-1 &
$ 06\h  56\m    39\fs    36$ &
$-67\degr 02' 16\farcs 8$ &
39 &
$0\fd 09081(18)$\\

Gaia DR3 5755874037751559424 &
$ 09\h  02\m    57\fs    71$ &
$-07\degr 59' 19\farcs 9$ &
$35$ &
$0\fd 15585(53)$\\

ATO J213.4592-29.8897 &
$ 14\h  13\m    50\fs    22$ &
$-29\degr 53' 23\farcs 1$ &
$38$ &
$0\fd 13879(43)$\\

3XLSS J231521.7-541842 &
$ 23\h  15\m    21\fs    72$ &
$-54\degr 18' 43\farcs 1$ &
$28$ &
$0\fd 14966(54) $\\

Gaia DR3 5499736649371768192 &
$ 06\h  27\m    51\fs    08$ &
$-53\degr 45' 17\farcs 7$ &
39 &
$0\fd 15838(53)$\\
\end{tabular}
\end{table*}

==> Tilted discs in six poorly studied CVs/tables/lookup_table.tex <==
\begin{table}
\centering
\caption{Tabular form of our derived $q(\varepsilon_-)$ relation for
$R_d = 0.9 - 1.1r_\text{tidal}$ using $r_\text{tidal}$ from \citet[Table
1]{Paczynski1977}.}
\label{tab:lookup_table}
\begin{tabular}{cccc}
\multirow{2}{*}{$|\varepsilon_-|$} & \multicolumn{3}{c}{$q(\varepsilon_-)$} \\[0.5ex]
\cline{2-4}\\[-1.5ex]
 & $0.9 r_\text{tidal}$ & $1.0 r_\text{tidal}$ & $1.1 r_\text{tidal}$
\\ \hline
0.006 & 0.039 & 0.032 & 0.031 \\
0.007 & 0.046 & 0.038 & 0.033 \\
0.008 & 0.053 & 0.044 & 0.038 \\
0.009 & 0.061 & 0.05  & 0.043 \\
0.010 & 0.069 & 0.057 & 0.048 \\
0.011 & 0.077 & 0.064 & 0.054 \\
0.012 & 0.086 & 0.071 & 0.060 \\
0.013 & 0.095 & 0.078 & 0.066 \\
0.014 & 0.104 & 0.085 & 0.071 \\
0.015 & 0.113 & 0.093 & 0.078 \\
0.016 & 0.124 & 0.101 & 0.084 \\
0.017 & 0.135 & 0.108 & 0.091 \\
0.018 & 0.145 & 0.117 & 0.097 \\
0.019 & 0.156 & 0.126 & 0.104 \\
0.020 & 0.167 & 0.135 & 0.110 \\
0.021 & 0.178 & 0.144 & 0.118 \\
0.022 & 0.191 & 0.153 & 0.126 \\
0.023 & 0.205 & 0.162 & 0.134 \\
0.024 & 0.218 & 0.171 & 0.142 \\
0.025 & 0.232 & 0.181 & 0.149 \\
0.026 & 0.246 & 0.193 & 0.157 \\
0.027 & 0.262 & 0.204 & 0.165 \\
0.028 & 0.279 & 0.216 & 0.173 \\
0.029 & 0.297 & 0.227 & 0.182 \\
0.030 & 0.314 & 0.239 & 0.192 \\
0.031 & 0.332 & 0.251 & 0.201 \\
0.032 & 0.352 & 0.265 & 0.211 \\
0.033 & 0.373 & 0.280 & 0.221 \\
0.034 & 0.393 & 0.295 & 0.231 \\
0.035 & 0.414 & 0.310 & 0.241 \\
0.036 & 0.436 & 0.324 & 0.251 \\
0.037 & 0.461 & 0.340 & 0.264 \\
0.038 & 0.487 & 0.358 & 0.277 \\
0.039 & 0.513 & 0.375 & 0.289 \\
0.040 & 0.539 & 0.392 & 0.302 \\
0.041 & 0.566 & 0.410 & 0.315 \\
0.042 &       & 0.427 & 0.328 \\
0.043 &       & 0.448 & 0.341 \\
0.044 &       & 0.470 & 0.356 \\
0.045 &       & 0.492 & 0.371 \\
0.046 &       & 0.514 & 0.386 \\
0.047 &       & 0.536 & 0.401 \\
0.048 &       & 0.558 & 0.415 \\
0.049 &       &       & 0.431 \\
0.050 &       &       & 0.449 \\
0.051 &       &       & 0.468 \\
0.052 &       &       & 0.487 \\
0.053 &       &       & 0.505 \\
0.054 &       &       & 0.524 \\
0.055 &       &       & 0.543 \\
0.056 &       &       & 0.562 \\
0.057 &       &       & 0.581
\end{tabular}
\end{table}

==> Tilted discs in six poorly studied CVs/tables/lookup_table_fit.tex <==
\begin{table}
\centering
\caption{Equation \eqref{eq:e_q_appendix_fit} fit coefficients $a$ and $b$ that approximate Table \ref{tab:lookup_table} data for different values of $R_d$. 
}
\label{tab:lookup_table_fit}
\begin{tabular}{cccc}
$R_d$ & $a$ & $b$ & $|\varepsilon_-|$ interval\\
\hline
$0.9 r_\text{tidal}$ & 0.155 & 1.706 & [0.006, 0.041] \\
$1.0 r_\text{tidal}$ & 0.182 & 1.694 & [0.006, 0.048] \\
$1.1 r_\text{tidal}$ & 0.210 & 1.680 & [0.006, 0.057]
\end{tabular}
\end{table}

==> Tilted discs in six poorly studied CVs/tables/shList.tex <==
\begin{table*}
\caption{List of CVs with discovered nSHs using the methods described
in Section~\ref{sec:Analysis}. All periodicities in this table
were measured on a Lomb-Scargle periodogram of range
0.125--16~\invday~and of ten-fold oversampling. All measured
$P_\text{prec}$ in this table agree within uncertainty with the expected
values by Equation~\eqref{eq:beat} using measured $P_\text{orb}$ and
$P_\text{nSH}$. Equatorial coordinates come from Gaia DR3 and are in
the J2000 epoch.}
\label{tab:shList}
\begin{tabular}{lrrcllll}
\multicolumn{1}{c}{Name} &
\multicolumn{1}{c}{RA} &
\multicolumn{1}{c}{Dec} &
\multicolumn{1}{c}{TESS Sector} &
\multicolumn{1}{c}{$P_\text{orb}$} &
\multicolumn{1}{c}{$P_\text{nSH}$} &
\multicolumn{1}{c}{$P_\text{prec}$} &
\multicolumn{1}{c}{$|\varepsilon_-|$}
\\ \hline
% \\[0ex] % Please replace if different stars need to be
%         %  separated by additional hspace

HBHA 4204-09 &
$ 21\h  07\m    52\fs    24$ &
$+44\degr 05' 42\farcs 0$ &
15, 16 &
$0\fd 14128(22)$ &
$0\fd 13657(22)$ &
$4\fd 11(18)$ & 
0.0333(22)

\\[0ex]
Gaia DR3 4684361817175293440 &
$ 00\h  49\m    59\fs    93$ &
$-76\degr 08' 27\farcs 5$ &
28 &
$0\fd 15401(53)$ &
$0\fd 14750(52)$ &
$3\fd 40(27)$ &
0.0423(48)

\\[0ex]

KQ Mon &
$ 07\h  31\m    21\fs    13$ &
$-10\degr 21' 49\farcs 4$ &
34 &
$0\fd 13456(40)$ &
$0\fd 12894(38)$ &
$3\fd 12(24)$ & 
0.0418(41)


\\[0ex]
SDSS J090113.51+144704.6 &
$ 09\h  01\m    13\fs    51$ &
$+14\degr 47' 04\farcs 7$ &
44 -- 46 &
$0\fd 14631(17)$ &
$0\fd 13991(17)$ &
$3\fd 198(70)$ &
0.0437(16)

\\[0ex]
Gaia DR3 5931071148325476992 &
$ 16\h  36\m    03\fs    63$ &
$-52\degr 33' 32\farcs 6$ &
39 &
$0\fd 14827(46)$ &
$0\fd 14248(43)$ &
$3\fd 57(30)$ &
0.0391(42)

\\[0ex]
{[}PK2008{]} HalphaJ103959 &
$ 10\h  39\m    59\fs    98$ &
$-47\degr 01' 26\farcs 3$ &
36, 37 &
$0\fd 1577(2)^\dagger$ &
$0\fd 15285(29)$ &
$4\fd 94(26)$ &
0.0308(22)
\\

\hline									
\end{tabular} 							
\par\hspace{10pt}
\raggedright
$^\dagger$Orbital period measured spectroscopically by \citet{Pretorius2008}.
\end{table*}

==> Tilted discs in six poorly studied CVs/tables/shmassratios.tex <==
\begin{table}
\centering
\caption{ Estimates of the mass ratio $q$ of Table \ref{tab:shList}
systems for disc radii $R_d=0.9r_\text{tidal}, 1.0r_\text{tidal}$, $1.1
r_\text{tidal}$ from \citet{Paczynski1977}, using the methods described
in Section~\ref{sec:Discussion_massratio}. Upper bounds of $q$ entering
the region of two-fold degeneracy are labeled with an asterisk.  
}
\label{tab:shmassratios}
\begin{tabular}{clll}
\multirow{2}{*}{Name} & \multicolumn{3}{c}{$q(\varepsilon_-)$} \\[0.5ex]
\cline{2-4}\\[-1.5ex]
 & $0.9 r_\text{tidal}$ & $1.0 r_\text{tidal}$ & $1.1 r_\text{tidal}$
\\ \hline

\multicolumn{1}{l}{HBHA 4204-09} &
0.38{\raisebox{0.5ex}{\tiny$^{+0.05}_{-0.05}$}} &
0.28{\raisebox{0.5ex}{\tiny$^{+0.03}_{-0.03}$}} &
0.22{\raisebox{0.5ex}{\tiny$^{+0.02}_{-0.02}$}} 
\\[0.2ex]


\multicolumn{1}{l}{Gaia-468436} &
0.60{\raisebox{0.5ex}{\tiny$^{+0.09^{*}}_{-0.13}$}} &
0.43{\raisebox{0.5ex}{\tiny$^{+0.10}_{-0.08}$}} &
0.33{\raisebox{0.5ex}{\tiny$^{+0.07}_{-0.06}$}} 
\\[0.2ex]


\multicolumn{1}{l}{KQ Mon} &
0.59{\raisebox{0.5ex}{\tiny$^{+0.11^{*}}_{-0.11}$}} &
0.42{\raisebox{0.5ex}{\tiny$^{+0.09}_{-0.07}$}} &
0.32{\raisebox{0.5ex}{\tiny$^{+0.06}_{-0.05}$}} 
\\[0.2ex]


\multicolumn{1}{l}{SDSS-090113} &
0.64{\raisebox{0.5ex}{\tiny$^{+0.04^{*}}_{-0.04}$}} &
0.46{\raisebox{0.5ex}{\tiny$^{+0.03}_{-0.03}$}} &
0.35{\raisebox{0.5ex}{\tiny$^{+0.02}_{-0.02}$}} 
\\[0.2ex]


\multicolumn{1}{l}{Gaia-593107} &
0.52{\raisebox{0.5ex}{\tiny$^{+0.11}_{-0.10}$}} &
0.38{\raisebox{0.5ex}{\tiny$^{+0.08}_{-0.07}$}} &
0.29{\raisebox{0.5ex}{\tiny$^{+0.06}_{-0.05}$}} 
\\[0.2ex]

\multicolumn{1}{l}{PK-103959}  &
0.33{\raisebox{0.5ex}{\tiny$^{+0.04}_{-0.04}$}} &
0.25{\raisebox{0.5ex}{\tiny$^{+0.03}_{-0.03}$}} &
0.20{\raisebox{0.5ex}{\tiny$^{+0.02}_{-0.02}$}} 
\end{tabular} 							
\end{table}
